TaxiNLI: Taking a Ride up the NLU Hill

Pre-trained Transformer-based neural architectures have consistently achieved state-of-the-art performance in the Natural Language Inference (NLI) task. Since NLI examples encompass a variety of linguistic, logical, and reasoning phenomena, it remains unclear as to which specific concepts are learnt by the trained systems and where they can achieve strong generalization. To investigate this question, we propose a taxonomic hierarchy of categories that are relevant for the NLI task. We introduce TAXINLI, a new dataset, that has 10k examples from the MNLI dataset (Williams et al., 2018) with these taxonomic labels. Through various experiments on TAXINLI, we observe that whereas for certain taxonomic categories SOTA neural models have achieved near perfect accuracies - a large jump over the previous models - some categories still remain difficult. Our work adds to the growing body of literature that shows the gaps in the current NLI systems and datasets through a systematic presentation and analysis of reasoning categories.

==> TaxiNLI 2020 10K/extra.tex <==
 \begin{table*}[!htpb]
  \resizebox{\textwidth}{!}{  
\begin{tabular}{|l|l|l|}
\hline
   & Synthetic Examples and Labels (E/C/N)                   & MNLI Examples and Labels (E/C/N)                                                                                                               \\ \hline
Lexical           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Anakin was compassionate. \\ H: Anakin was empathetic.\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: so it's stayed cold for the \underline{entire} week \\ H: It has been cold for the \underline{whole} week.\end{tabular} \\ \hline

Syntactic         & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Anakin was an excellent pilot. H: The \\ piloting skills of Anakin was as good as his \\singing.\end{tabular}                                           &   \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Those in Egypt, Libya, Iraq, and Yemen were \\eventually overthrown by secular nationalist revolutionaries.\\ H: Secular nationalist revolutionaries eventually \\overthrew them in Egypt and Libya.\end{tabular}                                                                                                                            \\ \hline
Factivity         &                                                                                                                                                                                         &                                                                                                                               \\ \hline
\multicolumn{3}{|c|}{\textbf{Logic}}                                                                                                                                                                                                                                                                                                                 \\ \hline\hline
Negation          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: Laurie has only visited Nephi, Marion has \\ only visited Calistoga. H:  Laurie didn’t visit \\ Calistoga.\end{tabular}                           &            \begin{tabular}[c]{@{}l@{}}{[}C{]} P: They \underline{post} loads of newspaper articles--Yahoo!\\ H:  Yahoo does \underline{not post} any articles from newspapers.\end{tabular}                                                                                                                   \\ \hline
Boolean           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Travis, Arthur, Henry and Dan have only \\ visited Georgia. H:  Dan didn’t visit Rwanda.\end{tabular}                                             &     \begin{tabular}[c]{@{}l@{}}{[}E{]} P:According to contemporaneous notes, \\at 9:55 the Vice President was still on the phone with the\\ President advising that three planes were missing \underline{and} one had hit\\ the Pentagon.\\ H:  The President called the Vice President to \\tell him the plane hit the Pentagon.\end{tabular}                                                                                                                          \\ \hline
Quantifier        & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Everyone has visited every place. H:  Virgil \\ didn’t visit Barry.\end{tabular}                                                                  &   \begin{tabular}[c]{@{}l@{}}{[}C{]} P: \underline{Some} travelers add Molokai and Lanai to their itineraries.\\ H:  \underline{No one} decides to go toMolokai and Lanai.\end{tabular}                                                                                                                             \\ \hline
Conditionals      & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Francisco has  visited Potsdam and if \\Francisco  has visited Potsdam then Tyrone has \\ visited Pampa. H:  Tyrone has visited Pampa\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Francisco has  visited Potsdam and if \\Francisco  has visited Potsdam then Tyrone has \\ visited Pampa. H:  Tyrone has visited Pampa\end{tabular}                                                                                                                              \\ \hline
Comparatives      & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: John \underline{is taller than} Gordon and Erik..., and \\ Mitchell is \underline{as tall as} John. H: Erik \underline{is taller than} \\ Gordon.\end{tabular}                        &      \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Load time is divided into elemental and coverage related load time.\\ H: The coverage related load time \underline{is longer than} elemental.\end{tabular}                                                                                                                         \\ \hline
%Monotonicity      & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: All black mammals saw exactly 5 \\ stallions who  danced. H: A brown \\ poodle saw exactly 5 stallions who danced.\end{tabular}           &                                                                                                                               \\ \hline
\end{tabular}
}
\caption{We provide a synthetic example and an an example from MultiNLI dataset that fall in each categories. For a full set of examples and definitions, please look at appendix.}
\label{tabexamples}
\end{table*}

\begin{table*}[!htpb]
  \resizebox{\textwidth}{!}{  
\begin{tabular}{|l|l|l|}
\hline
                  & Synthetic Examples and Labels (E/C/N)                                                                                                                                                   & MNLI Examples and Labels (E/C/N)                                                                                                               \\ \hline
    \multicolumn{3}{|c|}{\textbf{Reasoning}}                                                                       \\ \hline\hline
Relational        & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: \underline{Jack} and his \underline{brother} played cards. \\ H: The \underline{two siblings} played cards..\end{tabular}                                                             &   \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Actually, \underline{my sister} wrote a story on it. \\ H: \underline{My sibling} created a story about it. \end{tabular}                                                                                                                                                                  \\ \hline
Spatial  & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: The restaurant is just left of the shop,\\ opposite  the apartments. H: The restaurant is \\next to the shop.\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: At the eastern end of Back Lane and turning right,\\ Nicholas Street becomes Patrick Street, and in St. Patrick's\\ Close is St. Patrick's Cathedral .\\ H: Nicholas Street becomes Patrick Street after\\ turning left at the eastern end of Back Lane.\end{tabular}                                                                                                                              \\ \hline
Temporal          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: They worked in the fields only between\\ 3:30pm  and 4:40pm. H: They were hard at work \\ in the fields at 7:00pm.\end{tabular}                   &  \begin{tabular}[c]{@{}l@{}}{[}C{]} P: See you \underline{Aug. 12, or soon thereafter}, we hope.\\ H: The person told not to come \underline{until December}.\end{tabular}                                                                                                                             \\ \hline
Coreference       & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Jack found James annoying because of \\\underline{his}  constant meddling. H: \underline{Jack} was constantly \\ meddling with James\end{tabular}                         &    \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Acroseon the mountainside is another terrace on which \\imperial courtiers and dignitaries would sit while \\enjoying dance performances and music recitals on the \underline{hondo's broad terrace}.\\ H: There is a \underline{terrace} where musicians play.\end{tabular}                                                                                                                           \\ \hline
Causality       &\begin{tabular}[c]{@{}l@{}}{[}E{]} P:  John shot Mia in the leg. \\ H:Mia is hurt.\end{tabular}                                                                                                                              & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: A dozen minor wounds crossed his forearms and body. \\ H: The grenade explosion left him with a lot of wounds.\end{tabular}                                                                                                                               \\ \hline
\multicolumn{3}{|c|}{\textbf{Knowledge}}                                                                      \\ \hline\hline
World             & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: The church gathered in prayer. H: They \\ prayed to Allah.\end{tabular}                                                                           &                                                                                           
 \\ \hline
Taxonomic         & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: The ladybug ate part of the rose. \\ H: The insect ate part of the flower.\end{tabular}                                                           &                                                                                  \\ \hline   
\end{tabular}
}
\caption{In this table, we provide examples for the Reaosning and Knowledge categories. For a full set of examples and definitions, please look at appendix.}
\label{tabexamples2}
\end{table*}

==> TaxiNLI 2020 10K/sections/1_introduction.tex <==
\section{Introduction}


The Natural Language Inference (NLI) task tests whether a hypothesis (H) in text contradicts with, is entailed by, or is neutral with respect to a given premise (P) text. %~\cite{dagan2005pascal}. 
This 3-way classification task, popularized by \citet{bowman2015large}, which was in turn inspired by \citet{dagan2005pascal},  now serves as a benchmark for \textit{evaluation} of natural language \textit{understanding} (NLU) capability of models; for example, NLI datasets~\cite{bowman2015large,bowman2018-mnli} are included in all NLU benchmarks  such as GLUE and SuperGLUE \cite{wang2018glue}. These corpora, in turn, have been successfully used to train models such as BERT \cite{devlin2019bert} to achieve state-of-the-art (SOTA) performance in these tasks. Despite the wide adoption of NLI datasets, a growing concern in the community has been the lack of clarity as to \textit{which linguistic or reasoning concepts these trained NLI systems are truly able to learn and generalize} (see, for example~\cite{linzen-2020-accelerate} and \cite{bender-koller-2020-climbing}, for a discussion). Over the years, as models have shown steady performance increases in NLI tasks, many authors \cite{nie2019adversarial,kaushik2019learning} demonstrate steep drops in performance when these models are tested against adversarially (or counterfactually) created examples by non-experts.  \citet{Richardson2019ProbingNL} use templated examples to show trained NLI systems fail to capture essential logical (negation, boolean, quantifier) and semantic (monotonicity) phenomena.


%Marking a shift from logical entailment and following \cite{dagan2005pascal}, the authors of the NLI datasets relied on non-expert humans to determine \textit{entailment} of a premise, hypothesis pair.
%This enabled researchers  \cite{bowman2015large,bowman2018-mnli} to employ crowdsourcing to create several large corpora of NLI examples. 
 %and subsequent natural language understanding (NLU) benchmarks  such as GLUE \cite{wang2018glue} (a super-set of the NLI datasets). 
  %\footnote{Ideally, we are interested to know for which phenomenon (linguistic or logical), the systems achieve algorithmic strong generalization. For example, authors in \cite{xu2019can}, tests model's capability to represent dynamic programming class of problems. In this work, we aim to achieve the first step, i.e. identify all relevant phenomena and investigate which ones call for such explorations.}. 

    %Drawing our attention to the growing difference between quantified performance and our intuition, \cite{bender-koller-2020-climbing} cites the Chinese Room Experiment \cite{searle1980minds} and suggests that end-to-end tasks meant to test \textit{understanding} may only end up testing the input-output \textit{mimicking} capability. Authors in \cite{linzen-2020-accelerate} compared the current evaluation setup (NLI tasks, and benchmarks such as GLUE) as hill-climbing where the setup inadvertently favors large pre-trained models benefiting from fine-tuning; while keeping questions about reasoning capabilities and understanding largely un-answered. Most importantly, citing the limitations of crowd-sourced NLU datasets, \cite{bender-koller-2020-climbing} reminds us: 
    %\begin{quote}
     %     \textit{``there is no reason to assume that the distribution of language in the test data remotely resembles the distribution of real natural language"}
    %\end{quote}
    
    %Essentially, h
    Herein lie the central questions of our work: 1) what is the distribution of various categories of {\em reasoning tasks} in the NLI datasets? 2) which categories of tasks are rarely captured by current NLI datasets (owing to the nature of the task and the non-expert annotators)? 3) which categories are well-understood by the SOTA models? and 4) are there categories where Transformer-based architectures are consistently deficient? 
    %Our aim is two-fold: 1) augmenting the NLI task based evaluation setup to gain category-wise insights, 2) identifying under-represented and under-performing categories to influence better model building.  creating templated, synthetic or new crowdsourced examples, we focus on \textit{in-distribution} re-evaluation.  
    
    In order to answer these questions, we first discuss why performance-specific error analysis categories \cite{wang2018glue, nie2019adversarial}, and stress testing categories \cite{naik-etal-2018-stress} are inadequate. We then propose a taxonomy of the various reasoning tasks that are commonly covered by the current NLI datasets (Sec~\ref{sec:taxonomy}).  Next, we annotate 10,071 P-H pairs from the MNLI dataset~\cite{bowman2018-mnli} with the lowest level taxonomic categories, 18 in total (Sec~\ref{sec:taxinli}). Then we conduct various experiments and careful error analysis of the SOTA models---BERT and RoBERTa, as well as other baselines, such as Bag-of-words Na\"ive Bayes and ESIM, on their performance across these categories (Sec~\ref{sec:eval}). Our analyses indicate that while these models perform well on some categories such as linguistic reasoning, the performance on many other categories, such as those that require world knowledge or temporal reasoning, are quite poor. We also look into the embeddings of the P-H pairs to understand which of these categorical distinctions are captured well in the learnt representations, and which get conflated (Sec~\ref{sec:discussion}). Inline with our previous finding, we observe strong correlation between the level of clustering within the representation of the examples from a category, and the performance of the models for that particular category.
    
    
    
    %we augment the current accuracy-led evaluation setup to take a closer look at category-wise model performance. Lastly we identify under-represented and under-performing categories. % There have been works proposing performance-specific error analysis categories \cite{wang2018glue, nie2019adversarial}, and some generic categorization such as stress test types \cite{naik-etal-2018-stress}. However, most of these categories are dependent on the current training regime of deep learning and accuracy in the benchmark tasks, and  they do not provide a holistic understanding of a model's coverage of concepts.
    %In this paper, we aim to answer the first three questions and discuss how our solution may lead to answering the fourth question. We take a closer look at the model performance by establishing an umbrella taxonomic categorization and an accompanying dataset of annotated examples. 
    
    %Specifically, the contributions of this paper are threefold: First, we propose a detailed taxonomy capturing linguistic, logical and reasoning phenomena. Second, we introduce a new dataset, \textsc{TaxiNLI}, of NLI examples labeled by the reasoning tasks involved; And third, using \textsc{TaxiNLI}, we bring out certain reasoning categories that are difficult for the current models to solve.

    
    
    
    
    %We also include categories that are seldom represented in NLI datasets, but are interesting.
 %Next, using such categories, we employ a set of trained annotators to re-annotate a large fraction of MultiNLI examples (\textsc{TaxiNLI}). %To re-utilize already annotated large datasets, the examples are sampled from the MultiNLI dataset, and then re-annotated using our categories. 
      %We discuss our annotation framework in detail and make the examples, 
 
  %We also conclude the discussion by showing how some of these categories may warrant for capabilities of neuro-symbolic systems.  

==> TaxiNLI 2020 10K/sections/2_taxonomy.tex <==

%\section{Related Work}
%The NLI task represents a complex gamut of linguistic phenomena. 
%Digging deeper into the impressive performance of BERT (a Transformer-based architecture) in SNLI  \cite{bowman2015large}, authors \cite{poliak-etal-2018-collecting,gururangan2018annotation} showed that systems can easily exploit hypothesis-label correlation to achieve strong accuracy numbers.  Authors in \cite{glockner-etal-2018-breaking} showed that these trained systems struggle to perform simple lexical-level inferencing. Later for MNLI \cite{bowman2018-mnli}, similar issues such as above seems to repeat, as observed by \citeauthor{mccoy-etal-2019-right} (\citeyear{mccoy-etal-2019-right}). \citeauthor{Richardson2019ProbingNL} (\citeyear{Richardson2019ProbingNL}) observed that trained systems on SNLI and MNLI do not capture logical and semantic phenomenon. As the observations conflicted with the conclusions drwan from popular benchmark-based evaluation setup, it led to the following streams of research, namely 1) proposing new (or de-biased) datasets, 2) probing tasks for Transformer architectures, 3) post-hoc challenge datasets for trained NLI systems, and 4) stress-testing evaluation.

 
%Among newly proposed NLI datasets, Diverse NLI \cite{poliak-etal-2018-collecting} was one of the first, where authors synthetically recast existing NLU datasets into NLI task format. Due to the synthetic nature of the dataset, it has seen limited adoption. Recently, \cite{nie2019adversarial} created adversarial examples with the help of non-expert annotators playing games with SOTA NLI models. Our taxonomic evaluation setup complements adversarial datasets, as \citeauthor{linzen-2020-accelerate} (\citeyear{linzen-2020-accelerate}) mentions that non-adversarial evaluation paradigms are required to outline the true expectation from a system for a task. Additionally, counterfactually created datasets \cite{kaushik2019learning} showed huge performance drop in existing systems. They do not expose the linguistic aspects where the current systems had difficulty.


\section{A New Taxonomy for NLI}
\label{sec:taxonomy}
\subsection{Necessity for a New Taxonomy}
According to \citet{wittgenstein-1922}, ``Language disguises the thought'', and human beings try to gauge such thought from colloquial language using  ``complex silent adjustments''. The journey from lexicon and syntax of ``language'' to the aspects of semantics and pragmatics can be thought of as a journey that %\textit{form} to \textit{meaning} \cite{bender-koller-2020-climbing}, and this
portrays important milestones that an ideal NLU system should achieve. Irrespective of the order of such milestones\footnote{``For an infant, a foreigner, or an instant-message addict, context is more important than syntax'' \cite{sowa2010role}.}, we believe that NLU (and NLI) systems should be tested and analyzed with respect to fundamental linguistic and logical phenomena. Recently, different types of phenomena have been tested through 1) creating new datasets, 2) probing tasks, and 3) error-analysis categorizations. Researchers have created new datasets by recasting various NLU tasks to a large NLI dataset \cite{poliak-etal-2018-collecting}, eliciting counter-factual examples from non-experts by considering different lexical and reasoning factors \cite{kaushik2019learning}, and adversarial example \cite{nie2019adversarial} elicitation by letting non-experts come up with examples through interacting with SOTA systems. However, these datasets do not expose the linguistic aspects where the current systems have difficulty. Using the probing task methodology, researchers \cite{jawahar-etal-2019-bert,goldberg2019assessing} observed that BERT captures syntactic structure, along with some semantics such as NER, and semantic role labels \cite{tenney2019you}. However, BERT's ability to reason is questioned by the observed performance degradation in MNLI \cite{mccoy-etal-2019-right}. \citeauthor{linzen-2020-accelerate} (\citeyear{linzen-2020-accelerate}) also called for a pretraining-agnostic evaluation setup, where the setup is not limited to pre-trained language models. Our taxonomic categorization is meant to serve as a set of necessary inferencing capabilities that one would expect a competing NLI system to possess; thereby promoting more probing tasks along unexplored categories. %This is another reason, our taxonomic re-labeling of a subset of the MultiNLI may serve as a more detailed error analysis than a single numbered performance metric such as accuracy.
\begin{figure}%[!htb]
	\centering
    \includegraphics[width=0.48\textwidth]{figures/taxonomy.png} 
    % \resizebox{\columnwidth}{!}{
    % \input{taxinli.tikz}
    % }
    \caption{Taxonomic Categorization of the NLI task. 
    %\aalokcomment{TikZ version of this figure for better resolution, thanks to Saujas. Needs a little finetuning.}
    }
    \label{tax1}
\end{figure}


  
  Existing categorization efforts have centred around informing feature creation in the pre-Transformer era, and model-specific error analysis in more recent times. Previously, \cite{lobue2011types} enumerated the type of commonsense knowledge required for NLI. 
  Among recent error analysis efforts, the GLUE diagnostic dataset \cite{wang2018glue}, inference types for Adversarial NLI \cite{nie2019adversarial}, the new CheckList \cite{ribeiro-etal-2020-beyond} system and the Stress Tests \cite{naik-etal-2018-stress} are mentionworthy.  %Table \ref{tab:others} shows the categorizations proposed for NLI error analysis by \cite{nie2019adversarial,wang2018glue}. 
  As we attempted to group the categorizations in \citet{nie2019adversarial} and \citet{wang2018glue} into four high-level categories (lexical, syntactic, semantic, and pragmatic)\footnote{Table provided in Appendix}, we observe that there is a lack of consensus, non-uniformity and repetitiveness of these categories.  For example, the \textit{Tricky} label in \citet{nie2019adversarial} groups examples that involve ``wordplay, linguistic strategies such as syntactic transformations, or inferring writer intentions from contexts''; thereby spanning aspects of syntax and pragmatics. Similarly, \textit{Reference and Names} requires both reasoning and knowledge. The GLUE diagnostic categories \cite{wang2018glue} does not include interesting reasoning categories such as \textit{temporal}, and \textit{spatial}. 
  The stress types proposed by \citet{naik-etal-2018-stress} are specific to mostly lexical and some semantic corner cases. This is expected, as these categorizations are analysis-oriented and often dependent on the performance of a set of models in question. Here, we propose a taxonomic categorization that delineates a set of necessary uniform inferencing capabilities for the NLI task.
  
  %\somakcomment{Discussion/conclusion} Very recently, \cite{ribeiro-etal-2020-beyond} listed a set of universal phenomena and suggested to adopt behavioral testing of NLP models. Our categorization in-fact subsumes these categories, and our examples per categories \textsc{CheckList} can be thought of templates for testing minimal functionality testing (MFT) conditions for the NLI task.


% \begin{table}[!htpb]
% \resizebox{\columnwidth}{!}{ 
% \begin{tabular}{|l|l|l|}
% \hline
%                                                 & ANLI Inference Types                                           & GLUE Diagnostic                                                                                                                                                           \\ \hline
% Lexical                                         & \begin{tabular}[c]{@{}l@{}}Standard Inference\\ Lexical Inference\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Lexical Entailment\\ Morphological Negation\\ Factivity, Redundancy\end{tabular}                                                               \\ \hline
% Syntactic                                       & Tricky                                                                                                   & \begin{tabular}[c]{@{}l@{}}Syntactic Ambiguity, \\ Prepositional Phrase \\ Alternations: Active/Passive, \\ Genitives/Partitives, \\ Nominalization, Datives\end{tabular} \\ \hline
% \multicolumn{1}{|c|}{\multirow{4}{*}{Semantic}} & Standard Inference                                                                                       & \begin{tabular}[c]{@{}l@{}}Propositional Structure, \\ Intersectivity\\ Quantifiers, Restrictivity, \\ Quantification\end{tabular}                                        \\ \cline{2-3} 
% \multicolumn{1}{|c|}{}                          & \begin{tabular}[c]{@{}l@{}}Numerical, \\ Quantitative\end{tabular}                                       & Counting                                                                                                                                                                  \\ \cline{2-3} 
% \multicolumn{1}{|c|}{}                          & Reference and Names                                                                                      & \begin{tabular}[c]{@{}l@{}}Symmetry/Collectivity, \\ Coreference, Richer \\ Logical Structures\end{tabular}                                        \\ \cline{2-3} 
% \multicolumn{1}{|c|}{}                          & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Reference and Names\\ Reasoning about Facts\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Named Entities \\ Knowledge and \\ Commonsense\end{tabular}                                                                                    \\ \hline
% Pragmatics                                      & Tricky                                                                                                   & Ellipsis/Implicits                                                           \\ \hline
% \end{tabular}
% }
% \caption{We show existing NLI error-analysis categorizations proposed by the recent papers, and group them in higher-level categories.}
% \label{tab:others}
% \end{table}

  \begin{table*}[!htpb]
  \resizebox{\textwidth}{!}{  
% \begin{tabular}{llll}
\begin{tabular}{p{2.5cm}lp{2.5cm}l}
\toprule
            \textbf{Taxonomic Category} & \textbf{MNLI Examples }                                                                                                                                         &    \textbf{Taxonomic Category}           & \textbf{MNLI Examples }                                                                                                                                                   \\ \midrule
{\texttt{Lexical}}      & \begin{tabular}[c]{@{}l@{}}P: so it's stayed cold for the \underline{entire} week \\ H: It has been cold for the \underline{whole} week.\end{tabular}                                                                                                                                                                                             & {\texttt{Relational}}  & \begin{tabular}[c]{@{}l@{}}P: Actually, \underline{my sister} wrote a story on it. \\ H: \underline{My sibling} created a story about it.\end{tabular}                                                                                                                                                          \\ \hline
{\texttt{Syntactic}}    & \begin{tabular}[c]{@{}l@{}}P: Those in Egypt, Libya, Iraq, and Yemen were \\ eventually overthrown by secular nationalist revolutionaries.\\ H: Secular nationalist revolutionaries eventually \\ overthrew them in Egypt and Libya.\end{tabular}                                                                                                                                   & {\texttt{Spatial}}     & \begin{tabular}[c]{@{}l@{}}P: At the eastern end of Back Lane and turning right,\\ Nicholas Street becomes Patrick Street, and in St. Patrick's\\ Close is St. Patrick's Cathedral .\\ H: Nicholas Street becomes Patrick Street after\\ turning left at the eastern end of Back Lane.\end{tabular}                                               \\ \hline
{\texttt{Factivity}}    &                                \begin{tabular}[c]{@{}l@{}}P: The best place to view the spring azaleas is at the Azalea Festival\\ in the last week of April at Tokyo's Nezu shrine.\\ H:There is an Azalea Festival at the Nezu Shrine.\end{tabular}                                                                                                                                                                                                                                                                                                                                   & {\texttt{Temporal}}    & \begin{tabular}[c]{@{}l@{}}P: See you \underline{Aug. 12, or soon thereafter}, we hope.\\ H: The person told not to come \underline{until December}.\end{tabular}                                                                                                                                               \\ \hline
{\texttt{Negation}}     & \begin{tabular}[c]{@{}l@{}}P: They \underline{post} loads of newspaper articles--Yahoo!\\ H:  Yahoo does \underline{not post} any articles from newspapers.\end{tabular}                                                                                                                                                                          & {\texttt{Causal}}      & \begin{tabular}[c]{@{}l@{}}P: Acroseon the mountainside is another terrace on which \\ imperial courtiers and dignitaries would sit while \\ enjoying dance performances and music recitals on the \\ \underline{hondo's broad terrace}.\\ H: There is a \underline{terrace} where musicians play.\end{tabular} \\ \hline

{\texttt{Boolean}}      & \begin{tabular}[c]{@{}l@{}}P:According to contemporaneous notes, at 9:55 the Vice President \\ was still on the phone with the President advising that three planes \\were missing \underline{and} one had hit the Pentagon.\\ H:  The President called the Vice President to tell him the plane \\hit the Pentagon.\end{tabular} & \texttt{Coreference}       & \begin{tabular}[c]{@{}l@{}}P: A dozen minor wounds crossed his forearms and body. \\ H: The grenade explosion left him with a lot of wounds.\end{tabular}                                                                                                                                                                                         \\ \hline
{\texttt{Quantifier}}   & \begin{tabular}[c]{@{}l@{}}P: \underline{Some} travelers add Molokai and Lanai to their itineraries.\\ H:  \underline{No one} decides to go to Molokai and Lanai.\end{tabular}                                                                                                                                                                     & \texttt{World}       & \begin{tabular}[c]{@{}l@{}}P: In this respect, bringing Steve Jobs back to save Apple\\ is like bringing Gen.\\ H: Steve Jobs unretired in 2002.\end{tabular}                                                                                                                                                                                                                                             \\ \hline
{\texttt{Conditional}} & \begin{tabular}[c]{@{}l@{}}P: If the revenue is transferred to the General Fund, it is recognized \\as nonexchange revenue in the Government-wide consolidated \\ financial statements.\\ H: Revenue from the General Fund is not considered in financial statements\end{tabular}                                                                                                                                                                                                   & \texttt{Taxonomic} & \begin{tabular}[c]{@{}l@{}}P: Benson's action picture in Lucia in London \\(Chapter 8)- Georgie stepped on a beautiful \underline{pansy}. \\ H: Georgie crushed a beautiful \underline{flower} in Chapter 8 \\of Lucia in London.\end{tabular}                                                                              \\ \hline
\texttt{Comparative} & \begin{tabular}[c]{@{}l@{}}P: Load time is divided into elemental and coverage related load time.\\ H: The coverage related load time \underline{is longer than} elemental.\end{tabular}                     &             &                                                           \\ \bottomrule
\end{tabular}
}
\caption{For each category, we provide an example from the MNLI dataset. For a full set of synthetic examples and definitions, please look at appendix.}
\label{tabexamples}
\end{table*}

\subsection{Taxonomic Categories: Definitions and Examples}
In Figure \ref{tax1}, we present our taxonomic categorization. Our categorization is based on the following principles.  \underline{First}, we take a model-agnostic approach, where we work from the first principles to arrive at a set of basic inferencing processes that are required in NLI task. These include an unrestricted variety of linguistic and logical phenomena, and may require knowledge beyond text, thus providing us with the higher-level categories: \textit{linguistic}, \textit{logical} and \textit{knowledge}-based. \underline{Second}, we retain categories that are non-overlapping and sufficiently represented in NLI datasets. For example, for sub-categories under {\it linguistic}, we prune \textit{semantics} because necessary aspects are covered by \texttt{logical} and \texttt{knowledge}-based categories. We omit specific aspects of \textit{pragmatics} such as implicatures and pre-suppositions, as they are rarely observed in NLI datasets \cite{jeretic-etal-2020-natural}. \underline{Thirdly}, we aim to list a set of necessary sub-categories. For example, for logical deduction sub-categories, we take inspiration from \citet{davis2015commonsense}, who list the commonsense reasoning categories where systems have seen success.   \underline{Lastly}, since we aim to employ non-experts for collecting annotations, we decide to restrict further sub-division wherever the definitions get complicated, or pre-suppose certain expertise; for example the \texttt{lexical} category is not sub-divided further (as followed in \citet{wang2018glue}). Thus, we take a pragmatic approach that is theory neutral and does not warrant coverage of all reasoning tasks, though we do believe that the taxonomy is sufficiently deep and generic that allows systematic and meaningful analysis of NLI models with respect to their reasoning capabilities.

Next we define the categories. For a full set of examples, please see Table \ref{tabexamples}. 

% \begin{figure}[!htb]
% 	\centering
%     \includegraphics[width=0.48\textwidth]{figures/taxonomy.png} 
%     \caption{Taxonomic Categorization of the NLI task. }
%     \label{tax1}
% \end{figure}

\underline{High-Level Categories}: The \textbf{\texttt{Linguistic}} category represents NLI examples where the inference process to determine the entailment are internal to the provided text. We classify examples as \textbf{\texttt{Logical}} when the inference process may involve processes external to text, such as mapping words to percepts and reason with them \cite{sowa2010role}. \textbf{\texttt{Knowledge}}-based category represents examples where some form of external, domain or commonly assumed knowledge is required for inferencing. 

\textbf{\texttt{Linguistic}} category is further sub-divided into \texttt{lexical}, \texttt{syntactic}, and \texttt{factivity}.\\\noindent
1. \underline{\textbf{Lexical}}: This category captures P-H pairs where the text is almost the same apart from removal, addition or substitution of some lexical items. \textbf{Example}: P: Anakin was kind. H: Anakin was cruel.\\\noindent
2. \underline{\textbf{Syntactic}}:  \texttt{Syntactic} deals with examples where syntactic variations or paraphrases are essential to detecting entailment. \textbf{Example}: P: Anakin was an excellent pilot. H: The piloting skills of Anakin were excellent.\\\noindent
3. \underline{\textbf{Factivity}}:  Here the hypothesis contains an assumed fact from the premise, mostly an assumption about the existence of an entity or the occurrence of an action (inspired from \citet{wang2018glue}). \textbf{Example}: P: Padme recognized that Anakin was intelligent. H: Anakin was intelligent.

Based on commonalities, \textbf{\texttt{Logical}} categories are grouped under ``Connectives''. ``Mathematical'' and ``Deduction''. \\\noindent
1. \underline{\textbf{Connectives (Negation, Boolean, Quantifiers}}, \underline{\textbf{Conditionals, Comparatives)}}: We group the logical categories \texttt{negation, boolean, quantifier, conditional} and \texttt{comparative} \cite{salvatore2019logical} under the ``Connectives'' label. \texttt{Negation} applies when P negates one (or more) of the facts in H. We apply the category \texttt{boolean} when P is a set of statements connected by \textit{or, and} and H talks about one of the statements. \texttt{Quantifier} is applied when P or H requires understanding of words denoting existential or universal quantifiers. Similarly, \texttt{conditional} is applicable where P or H has conditional statements. If P (or H) compares entities via comparative phrases, then we label it as \texttt{comparative}. \textbf{Examples}: (\texttt{boolean} and \texttt{negation}) P: Jar Jar, R2D2 and Padme only visited Anakin’s house. H: Jar Jar Binks didn’t visit Anakin’s shop.\\\noindent
2. \underline{\textbf{Mathematical (Counting, Arithmetic)}}: This group of categories is concerned with examples that require mathematical reasoning. For brevity, we concentrate on examples that require counting and simple arithmetic operations. However, we observed exceedingly low number of examples in this category group from our pilot study on SNLI and MNLI, and hence we remove these from our final annotations.\\\noindent
%\textbf{Examples}: (\texttt{Counting}): P: Nellie has only visited Carrie, Billie, John, Mike, Thomas,  and Arthur. H: Nellie has visited more than 10 people. More in appendix.\\\noindent
3. \underline{\textbf{Deductions (Relational, Spatial, Temporal}}, \underline{\textbf{Causal, Coreference)}}: Motivated by predicate logic, success of qualitative representation and reasoning in dealing with temporal and spatial reasoning \cite{gabelaia2005combining}, and causality \cite{pearl2009causality}, we list \texttt{relational}, \texttt{temporal, spatial} and \texttt{causal} under ``Deductions''. The \texttt{relational} reasoning stands for the requirement to perform deductive reasoning using relations present in text. \texttt{Spatial} (and \texttt{temporal}) denotes reasoning using spatial (and temporal) properties of objects represented in text.  We also consider language-inspired reasoning categories such as co-reference resolution, which is known to often require event-understanding \cite{ng2017machine} beyond superficial cues. \textbf{Example}: (\texttt{relational}) P: The lamp was working properly. H: The lightbulb from the lamp was not functioning.

Lastly, we define two sub-categories under \textbf{\texttt{Knowledge}}, namely \texttt{world} and \texttt{taxonomic}.\\\noindent
1. \underline{\textbf{World}}: Examples that require knowledge about named entities, knowledge about historical, current events; and domain-specific knowledge. \textbf{Example}: (\texttt{world}) P: Michelle Obama stayed in the White House during 2009-17. H: Michelle was living in the White House legally during 2009. \\\noindent
2. \underline{\textbf{Taxonomic}}: Examples that require taxonomies and hierarchies. For example, \textit{IsA, hasA, hasProperty} relations. \textbf{Example}: (\texttt{taxonomic}) P: Norman hated all musical instruments. H: Norman loves the piano.

Note that presence of a certain lexical trigger for a category (such as negation) does not warrant the labeling with the category, unless understanding of that concept is invoked in the deduction process.

%The examples in the NLI datasets represent a complex gamut of linguistic phenomena.
%To categorize them in a model-agnostic way, we first look towards NLU in general and then filter infrequent categories based on pilot studies on NLI datasets (SNLI, MNLI). Holistic understanding of text written or spoken in natural language goes beyond the essential components of a language such as its lexicon, syntax and grammar. It naturally includes semantics. According to John Sowa \cite{sowa2010role}, semantics concerns with understanding ``the link from words to the concepts they express''; or ``the link from concepts to percepts of objects and actions upon them''. Such semantics, also concerns with \textit{reasoning} about objects and actions, often naturally concerning concepts external to text (\textit{knowledge}). As natural language is meant for communication, many aspects of pragmatics become important for a speaker and listener to converse successfully. Similar to \cite{jeretic-etal-2020-natural}, we observe that most elements of pragmatics such as motivation (affect etc.) and social interaction (speech acts, implicatures) are rarely captured by the large NLI datasets. %, provided the nature of their annotations. 
%Some aspects such as speech acts and implicatures are captured by code-mixed conversational NLI datasets \cite{khanuja2020new}; but they are out of scope of our work. Hence the top level interesting categories are: \texttt{lexical, syntactic,} and \texttt{semantic}. 

  %We start with \texttt{lexical} to capture P-H pairs where the text is almost the same apart from removal, addition or substitution of some words. \texttt{Syntactic} deals with examples where syntactic variations or paraphrases are essential to detecting entailment.
  %For us, the largest category is \texttt{semantic}, which we further divide into: \texttt{logic, mathematical, reasoning and knowledge}. This category is relevant as authors in \cite{bender-koller-2020-climbing,niven-kao-2019-probing} point out that current systems do not capture many aspects of \textit{meaning} such as reasoning which are inherently required for \textit{understanding}. Similar to previous work \cite{salvatore2019logical}, \texttt{Logic} deals with a set of surface logical connectives such as boolean (and/or), negation, quantifiers ($\forall, \exists$), conditionals (if/then) and comparatives (as tall as, taller than). We do not consider Monotonicity separately, as according to \cite{angeli2014naturalli} it captures many types of entailment and contradiction. On the other hand, the monotonic lexical relations (external to text) and types of reasoning it requires are captured by our \texttt{Reasoning} and \texttt{Knowledge} categories. 
  
  %\texttt{Mathematical} category concerns with examples that require mathematical reasoning. For brevity, we concentrate on examples that require counting and simple arithmetic operations. However, a pilot study on SNLI and MNLI showed that number of examples requiring such reasoning is limited ($14$ out of $350$). \texttt{Reasoning} category represents different types of reasoning. We consider categories representing some fundamental reasoning concepts such as relational, and causal; and modal logics such as spatial and temporal. The \texttt{relational} reasoning stands for the requirement to perform inductive and deductive reasoning using relations present in text. As \texttt{relational} is a large category, we do not consider categories such as taxonomic reasoning separately \cite{davis2015commonsense}. We also consider language-inspired reasoning categories such as co-reference resolution. \texttt{Spatial} (and \texttt{temporal}) denotes reasoning using spatial (and temporal) properties of objects represented in text. For \texttt{Knowledge}, we take inspiration from the GLUE diagnostic categories \cite{wang2018glue} and consider two clear high-level categories: world knowledge which is explicitly stated, and commonsense which is implicitly understood or inferred. In Table \ref{tabexamples}, we provide a few examples for each category. The complete definitions of the categories and more examples will be available in the appendix. %\todocomment{We need good examples from MultiNLI and synthetic ones as well.}
  


==> TaxiNLI 2020 10K/sections/3_taxinli.tex <==
\section{TaxiNLI: Dataset Details}
\label{sec:taxinli}

We present TaxiNLI, a dataset collected based on the principles and categorizations of the aforementioned taxonomy. We curate a subset of examples from MultiNLI \cite{bowman2018-mnli} by sampling uniformly based on the entailment label and the domain. We then annotate this dataset with fine-grained category labels.  %\somakcomment{We do not need this: Our dataset contains fine-grained category annotations for a subset of datapoints from MultiNLI \cite{bowman2018-mnli}.}

\subsection{Annotation Process}
% \somakcomment{Pratik: 
%  i) Pilot Study Metrics and Learning: time taken, perceived correctness per category, which categories were confusing and what did we do, ii) annotator training period Details, iii) Annotation period metrics such as annotator accuracy and IAA etc. 
%  }
 %\subsubsection{Annotation Framework}
 
%\somakcomment{The first paragraph pf the section did not and this one can be merged as shown above: \textbf{Premise-Hypothesis Data:} We first sampled from MultiNLI, sampling uniformly based on entailment label and domain. We subsequently used this data for annotation. 
%\\}

%\somakcomment{Please use \paragraph{}, not \textbf{}}
\paragraph{Task Design} For large-scale data collection, our aim was to propose an annotation methodology that is relatively flexible in terms of annotator qualifications, and yet results in high quality annotations. To employ non-expert annotators, we designed a simplified guideline (questionnaire/interface) for the task, that does not pre-suppose expertise in language or logic. %as we believe that this task can be doesn't require linguists as annotators. 
As an overhead, the guideline requires a few rounds of one-on-one training of the annotators. Because it is expensive to perform such rounds of training in most crowdsourcing platforms, we hire and individually train a few chosen annotators.
%It is an easily explainable task, which requires a few rounds of training. This is also why we did not go with crowdsourcing, because one-to-one training for the annotators would be cumbersome. Thus, we designed %\somakcomment{since we are leaving it out, noone is going to know and care. So commenting this would be best.}\footnote{The designing and narrowing of the annotation process was complicated, which brought us additional insights in terms of how to conduct this task. However, in the interest of space, we are leaving this out.} 
% We design a questionnaire/interface which was suitable for non-experts. 
Upon conducting the previously-discussed pilot study and using the given feedback, we created a hierarchical questionnaire which first asked the annotator to do the NLI inference %(whether hypothesis was true/false/can't say with respect to the premise) 
on the P-H pair, and then asked targeted questions to get the desired category annotations for the datapoints. The questionnaire is shared in the Appendix. 


%We also received feedback about the added difficulty of the category annotation for the `neutral' examples. 
For the MNLI datapoints with `neutral' gold labels, we realized, through observation and annotator feedback, that annotating the categories were difficult, as sometimes the hypotheses could not be connected well back to their premise. Hence, we created 2 questionnaires, one for the `entailment/contradiction' examples, and one for `neutral' examples. For the entailment/contradiction examples, We collected binary annotations for each of the 15 categories in our NLI taxonomy, for datapoints in MNLI which had `entailment' or `contradiction' as gold labels.  %To resolve this, we introduced three more annotations, therefore simplifying the complicated nature of `neutral' examples. 
To resolve this, for the `neutral' examples we specifically %the annotators that each example had `neutral' inference, and 
asked them whether the premise and hypothesis were discussing 1) the same general topic (politics, geology, etc.), and if so, 2) had the same subject and/or object of discussion (Obama, Taj Mahal, etc.). If the response to 2) was `yes', then they were asked to provide the category annotations as previously defined. 

\paragraph{Annotator Training/Testing} We first tested our two annotators by asking them to do inference on a set of randomly selected premise-hypothesis pairs from MultiNLI. This was to familiarize them with the inference task. After giving the category annotation task, we also continuously tested and trained the two annotators. After a set of datapoints were annotated, we reviewed and went through clarification and feedback sessions with the annotators to ensure they understood the task, and the categories, and what improvements were required. More details are provided in the Appendix. 
 
 %\paragraph{Annotation Platform Choice, Time and Cost} Provided the nature of the task, we had three possible choices: using 
 
 \subsubsection{Annotation Metrics}
 Here, we assess the individual annotator performance and inter-annotator agreement. Since, automated metrics for individual complex category annotations are hard to define, we use an indicative metric that matches the annotated inference label with the gold label, i.e., their \textbf{inference accuracy}.
 %Finding an automatic metric for annotator performance is difficult, especially in a complicated task as this. An indicative metric we used was checking the annotated inference label with the gold label, essentially their \textbf{inference accuracy}. 
 %In order to view improvement over annotation performance, We tracked the accuracy for each annotator over subsequent batches of data that they annotated. 
 %\somakcomment{We are not reporting these things. At best these should be footnote and appendix. Another automatic indicator we looked at was average number of category annotations per datapoint, and average number of annotations per category. Although this wasn't necessarily an indicator of annotator ability, it prompted us to regroup with the annotators in the case if the annotations were especially scarce, or if there were any particular confusing categories.} 
 We also calculated inter-annotator agreement between the two annotators for an overlapping subset of 600 examples. For agreement, we use the Fleiss' Kappa ($\kappa$) \cite{fleiss}. We also compute another simple statistic, namely the `IOU' (Intersection-Over-Union) of categories per datapoint, defined as:
 $IOU = \frac{1}{N}\sum_{i=1}^{N}{\frac{|{C_{A1}^{i}}\cap{C_{A2}^{i}}|}{|{C_{A1}^{i}}\cup{C_{A2}^{i}}|}},$ where $C_{Ai}^{j}$ are the category annotations for Annotator $i$ for datapoint $j$, averaged over total datapoints $N$. 
 Looking at the category-wise Fleiss' $\kappa$ values in Fig. \ref{fig:iaa_categories}, we observe that there are promising levels of agreement in most of the categories except \texttt{syntactic}, \texttt{relational}, and \texttt{world}. We observe the average inference accuracy (86.7\%) is high despite known issues in MNLI example ambiguity. Similarly, both the average Fleiss' $\kappa$ (\textbf{0.226}) and the IOU metric (\textbf{0.241}) suggest an overall reasonable inter-annotator agreement.
 
\begin{figure}%[htb!]
	\centering
    \includegraphics[width=0.5\textwidth]{figures/iaa_values.png}
    \caption{Inter-annotator Agreement (IAA) values between the two annotators, plotted category-wise.}
    \label{fig:iaa_categories}
\end{figure}

% \begin{table}[!h]
% % \small
% \centering
% \begin{tabular}{|l|l|}
%       \hline
%       \textbf{Annotator Metric} &  \\
%       \hline
%       Average Inference Accuracy & 86.7\%\\
%       \hline
%       Average Fleiss $\kappa$ & 0.226 \\
%       \hline
%       IOU & 0.241   \\
%       \hline
% \end{tabular}
% \caption{Annotator Metrics. The Average Inference Accuracy is averaged over all the annotated datapoints, and the Fleiss $\kappa$ and $IOU$ are over a subset that has been annotated by both annotators.}
% \label{tab:taxinlistats}
% \end{table}

 %\somakcomment{Annotation accuracy, IAA tables/graphs}
%\subsubsection{Lessons from Pilot Study}
%\subsubsection{Deployment}
\subsection{Dataset Statistics}

Each datapoint in TaxiNLI\footnote{The dataset is available for download from \url{https://github.com/microsoft/TaxiNLI}.} consists of a premise-hypothesis pair, the entailment label, and binary annotations for 18 features. 15 features correspond to the 15 categories discussed in the taxonomy, and 3 additional features for the `neutral' gold label datapoints based on same general topic, same subject, and same object. The statistics are listed in Tab. \ref{tab:taxinlistats2}.

\begin{table}[!h]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ll}
      \toprule
    %   Statistic&\\
    %   \midrule
      Total datapoints& 10,071 \\
      \midrule
      \multirow{2}{*}{
        Datapoints overlapping with MNLI
      } 
        % \begin{tabular}[l]  33087 (Same general topic),\\\hline 2843 (Same object),\\\hline 877 (Same subject) \end{tabular} \\
        & 2343
        (train) \\
        &7728 (dev)  \\
      \hline
      Avg. datapoints per domain& $1007.1$ \\
      \hline
      Datapoints per NLI label & 3375 (C), 3201 (N), 3495 (E) \\
      \hline
      Avg. categories per datapoint & $1.6$ \\
      \hline
      \multirow{3}{*}{
        Neutral example characteristics
      } 
        % \begin{tabular}[l]  33087 (Same general topic),\\\hline 2843 (Same object),\\\hline 877 (Same subject) \end{tabular} \\
        & 3087 (Same general topic),\\ 
        & 2843 (Same object),\\
        & 877 (Same subject) \\
      \bottomrule
\end{tabular}}
\caption{TaxiNLI Statistics}
\label{tab:taxinlistats2}
\end{center}
\end{table}

\paragraph{Categorical Observations} From our annotations, we observe that inferencing each MNLI example requires about 2 categories. Fig.~\ref{fig:categories_freq} shows the distribution of categories in the TaxiNLI dataset. We see that a large number of P-H pairs in MNLI require \texttt{lexical} and \texttt{syntactic} knowledge to make an inference; whereas the challenges of \texttt{relational}, \texttt{spatial}, and \texttt{taxonomic} for inference are not adequately represented. There is a large proportion of examples in the \texttt{syntactic} category which have the `entailment' label, and a large proportion of \texttt{negation} examples have the `contradiction' label. Additionally, many `neutral' examples were classified as requiring \texttt{causal} knowledge. The feedback session with annotators revealed that there were many `neutral' examples where the hypothesis was essentially an unverifiable intent or detail of a certain action mentioned in the premise. An example is ``\textbf{P: }\textit{Another influence was that patrician politician Franklin Roosevelt, who was, like John D. Rockefeller, the focus of Nelson's relentless sycophancy and black-belt bureaucratic infighting.} \textbf{H: }\textit{Nelson targeted Roosevelt in order to gain political favor.}".
\begin{figure}%[htb!]
	\centering
    \includegraphics[width=0.48\textwidth]{figures/category_plot_split.png}
    \caption{The number of datapoints annotated with each category, split by the gold label of the datapoints. For \texttt{taxonomic}, the gold label split is 9(E)/7(C)/3(N).}
    \label{fig:categories_freq}
\end{figure}

\paragraph{Categorical Correlations} Fig.~\ref{categorical_correl} shows correlations among categories in our dataset. We observe that most categories show weak correlation in the MNLI dataset, hinting at a possible independence of categories with respect to each other. Relatively stronger positive correlations are seen between \texttt{boolean}-\texttt{quantifier}, and \texttt{boolean}-\texttt{comparative} categories. We specifically looked at the genre-wise split of datapoints containing \texttt{boolean}-\texttt{quantifier} and saw that nearly 25\% of them came from the `telephone' genre of MNLI. An example is ``\textbf{P: }\textit{have that well and it doesn't seem like very many people uh are really i mean there's a lot of people that are on death row but there's not very many people that actually um do get killed} \textbf{H: }\textit{Most people on death row end up living out their lives awaiting execution.}". \texttt{Factivity}, on the other hand, is negatively correlated with almost all the other categories, except \texttt{world}, which means P-H pairs labeled with \texttt{factivity} typically have no other categories marked. % \somakcomment{we can leave out the speculative statements, i.e. future work for now. } A more detailed qualitative analysis on genre-wise correlations may bring out interesting properties of different domains, and what category knowledge they bring to the data.

\begin{figure}[htb!]
	\centering
    \includegraphics[width=0.5\textwidth]{figures/category_correlation.png}
    \caption{The correlation matrix between the taxonomic categories. }
    \label{categorical_correl}
\end{figure}


==> TaxiNLI 2020 10K/sections/4_reevaluation.tex <==
\section{(Re)Evaluation of SOTA Models}
\label{sec:eval}

%In this work, we propose a taxonomy of categories and introduce the \textsc{TaxiNLI} dataset with NLI examples annotated with taxonomic categories. 
 We re-evaluate two Transformer-based and two standard baseline machine learning models on \textsc{TaxiNLI}, under the lens of the taxonomic categories. %we design experiments to answer the following: I) do some categories remain consistently harder as neural architectures got \textit{stronger}?; II) does Pre-trained language models come packed with knowledge of the proposed categories?
As baselines, we choose BERT-base \cite{devlin2019bert}, and RoBERTa-large \cite{liu2019roberta} as two state-of-the-art NLI systems. For our experiments, we use the pre-trained {BERT-base} and RoBERTa models from HuggingFace's Transformers implementation \cite{Wolf2019HuggingFacesTS}. As pre-Transformer baselines, we use the bidirectional LSTM-based Enhanced Sequential Inference model (ESIM) \cite{chen-etal-2017-enhanced}. We also train a Naive Bayes (NB) model using bag-of-words features for the P-H pairs after removing stop words\footnote{Using NLTK's \texttt{RTEFeatureExtractor}}.

\subsection{\textsc{TaxiNLI} Error Analysis}
We report the NLI task accuracy of the baseline systems on the MNLI validations sets in Table \ref{tab:nliacc}.
The systems are fine-tuned on the MNLI training set using the procedures followed in \citet{devlin2019bert,liu2019roberta,chen-etal-2017-enhanced}. 
\begin{table}[!htpb]
\resizebox{\columnwidth}{!}{
\begin{tabular}{rllll}%{|l|l|l|l|l|}
\toprule
      \textbf{MNLI-dev} & \textbf{NB} & \textbf{ESIM} & {\bf BERT$_\textsc{base}$} & \textbf{RoBERTa$_\textsc{large}$} \\ \midrule
{Matched} &  51.46  &     72.3   &  84.7         &   92.3      \\ %\hline
{Mismatched} & 52.31 &   72.1   &   84.8        &   90.0      \\ \bottomrule
\end{tabular}
}
\caption{MNLI-validation set accuracy.}
\label{tab:nliacc}
\end{table}

We evaluate the systems on a total of 7.7k examples, which are in the intersection of \textsc{TaxiNLI} and the validation sets of MNLI. %In Fig.~\ref{acc}, we plot the category-wise probability for correct prediction for each model. 

Figure \ref{acc} shows
for each category $c_i$, the normalized frequency for a model predicting an NLI example of that category accurately, i.e., $\frac{\#c_i=1,correct=1}{\#c_i=1}$. 
% From the resulting Figure \ref{acc}, w
We observe that compared to NB, the improvements in BERT have been higher in \texttt{lexical, syntactic} categories compared to others. Improvements in ESIM compared to NB show a very similar trend, and show for knowledge categories the improvements are negligible. ESIM shows largest improvement on \texttt{negation}.
\begin{figure}[htb!]
	\centering
    \includegraphics[width=0.48\textwidth]{figures/category_wise_accuracy1f.png}
    % \includegraphics[width=0.48\textwidth]{figures/frequentist.png}
    \caption{
        The normalized frequency of the systems predicting an example correctly, provided a category. 
    }
    \label{acc}
\end{figure}


% Since, examples are annotated with multiple categories, we capture the dependencies by defining a Bayesian Network (BN) where, each category (a boolean random variable) has a directed edge to the \textit{correct} node (representing correctness of prediction)\footnote{Additionally, we attempted to learn a Bayes Net from the data using \texttt{bnlearn} package. But the limited number of observations yield non-intuitive results.}. We learn the parameters by fitting this BN to the observed data. In Figure \ref{acc2}, we see from the Bayesian estimate again that, the improvements by BERT in categories such as \texttt{relational} reasoning has been low. It also shows, that there is a sharp decrease in accuracy for examples requiring the use of taxonomic (commonsense) knowledge. However, RoBERTa improves over NB and ESIM by large margins, albeit non-uniformly. %From both measures\footnote{The conditional probabilities from BN are calculated using \texttt{cpquery()} method with logical sampling, $10^6$ samples and averaging multiple runs.}, we see that RoBERTa improves on BERT-base for all categories. However, as the Bayesian estimate shows, the performance for \texttt{reasoning} and \texttt{commonsense} knowledge category remains consistently low. %that the trends per category remain similar for BERT-base and RoBERTa. 
% %It also shows that improvements in \texttt{syntactic} and \texttt{lexical} are the highest. The Bayesian estimate shows that the improvements in reasoning categories are low. It further shows that the commonsense knowledge category significantly suffers related to others. %, which is expected since for us this category consists of commonsense relations as well. 
% %Though the \texttt{causal} category seems to demonstrate higher performance, we believe it is due to the presence of multiple MNLI examples that contain superficial cues such as \textit{causes, because, reason of}. 


% \begin{figure}[htb!]
% 	\centering
%     \includegraphics[width=0.5\textwidth]{figures/category_wise_accuracy2.png}
%     \caption{We show a Bayesian Estimate of $P(correct=1|category=1)$ for different systems. }
%     \label{acc2}
% \end{figure}


==> TaxiNLI 2020 10K/sections/5_confounding.tex <==
\subsection{Factor Analysis}
\label{sec:confound}
%Since dependencies among categorical labels and prediction correctness are ignored by the frequentist method, we first calculate Pearson's Correlation between these variables. In Figure \ref{correl}, we see that for RoBERTa accurate predictions, there is relatively strong correlation with lexical, syntactic and negation categories. For other categories, correlation seem to be lower.
In order to quantify the precise influence of the category labels on the prediction of the NLI models, we probe into indicators and confounding factors using two methods: linear discriminant analysis (LDA) and logistic regression (LR).
We use indicators for each category (0 or 1) and for two potential confounding variables (lengths of P,{H}), to model the correctness of prediction of the NLI system.
The coefficients of these analyses on BERT are shown in Fig~\ref{fig:factor}.
% , we show the coefficients obtained from LDA and LR features (categories) needed for classifying BERT's prediction ability 
The values for RoBERTa follow a similar trend, and are presented in the appendix. 
%For the discriminant analysis, we plot the linear discriminant coefficients and regression coefficients for each feature. We observe that lexical, syntactic, factivity and some \textit{Connective} categories has the most significant discriminating power for determining BERT's correct prediction ability.
We see that presence of certain taxonomic categories strongly influence the correctness of prediction. 
As we found in the analysis presented in Sec.~\ref{sec:eval},
we observe that {\tt syntactic}, {\tt negation}, and {\tt spatial} categories are strong indicators of correctness of prediction. % by BERT.
On the other hand, {\tt conditional}, {\tt relational}, {\tt causal}, {\tt coreference} are harder to predict accurately.
Sentence length does not play a significant role.

We also make an observation for categories such as {\tt lexical, syntactic}, where the proportion of a single NLI label is high, also correlated with a high prediction accuracy (Fig.~\ref{fig:factor}).

%  To quantify this observation, we computed NLI label entropy for each category, and correlated it with LDA/LR coefficients for that category. the high ((negative)) correlation shows the low entropy implies a positive coefficient, which might mean in certain cases, identifying that category is itself very helpful to get the prediction right.

% NLI hardness over our taxonomy,
% we also compare with the NLI label-wise constitution of taxonomic categories (from Fig. \ref{fig:categories_freq}). 
% We observe a similar trend: for categories where there is a large share of some NLI label, such categories ({\tt syntactic}---entailment, {\tt negation}---contradiction) likely lead to correct classification into that NLI label merely if present. For other categories that are more evenly distributed ({\tt lexical}, {\tt factivity}), we observe they are not indicative of correctness by themselves. Interestingly, {\tt causal}, despite being dominated by the neutral NLI label, seems to be an unhelpful predictor, with similarly a comparatively poor performance in Fig~\ref{acc}; indicating that categories such as {\tt causal, coreference} are intrinsically harder.

\begin{figure}%[htb!]
	\centering
    \includegraphics[width=.48\textwidth]{figures/factor.png}
    \caption{
        Coefficients obtained through Linear Discriminant Analysis (LDA) and Logistic Regression (LR) to model the correctness of NLI prediction by BERT, given taxonomy categories and possible confound variables.
        Significant LR coefficients: 
        {\tt syntactic**}, {\tt negation***, boolean*}, {\tt causal***, world***}, {\tt Length2**}; % NEW data (but same significance)
        % {\tt syntactic**}, {\tt negation***, boolean*}, {\tt causal***, world***}, {\tt Length2**}; 
        where $p$ value is smaller than: 0.001***, 0.01**, 0.05*.
    }
    \label{fig:factor}
\end{figure}


==> TaxiNLI 2020 10K/sections/6_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\definecolor{neutral}{rgb}{1.0, 0.0, 1.0}
\definecolor{entailment}{rgb}{0.75, 0.75, 0.75}
\definecolor{contradiction}{rgb}{0.96, 0.87, 0.7}

\newcommand{\rulesep}{}%\unskip\ \vrule\ }

\begin{figure*}[htb!]
	\centering
	\begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/bbu-mnli+lexical_layer3.png}
        \caption{{\tt Lexical} coloured at BERT$_{\rm BASE}$ layer 3}
    \end{subfigure}%
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/bbu-mnli+logic_layer6.png}
        \caption{{\it Connectives} coloured at BERT$_{\rm BASE}$ layer 6}
    \end{subfigure}
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/bbu-mnli+syntactic_layer11.png}
        \caption{{\tt Syntactic} coloured at BERT$_{\rm BASE}$  layer 11}
    \end{subfigure}
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/bbu-mnli+reasoning_layer12.png}
        \caption{{\it Deductions} coloured at BERT$_{\rm BASE}$ layer 12}
    \end{subfigure}
    %
    %
    %
    % ROBERTA
    %
    %
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/roberta+lexical_layer1.png}
        \caption{{\tt Lexical} coloured at RoBERTa$_{\rm LARGE}$ layer 1}
    \end{subfigure}%
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/roberta+logic_layer19.jpg}
        \caption{{\it Connectives} coloured at RoBERTa$_{\rm LARGE}$ layer 19}
    \end{subfigure}
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/roberta+knowledge_layer21.png}
        \caption{{\it Knowledge} coloured at RoBERTa$_{\rm LARGE}$  layer 21}
    \end{subfigure}
    ~ \rulesep ~
    \begin{subfigure}[t]{0.47\columnwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/tsne/roberta+reasoning_layer21.jpg}
        \caption{{\it Deductions} coloured at RoBERTa$_{\rm LARGE}$ layer 21}
    \end{subfigure}
    % \caption{Caption place holder}
    % \includegraphics[width=\textwidth]{figures/tsne-roberta-bert.jpg}
    \caption{Layer-wise 2D t-SNE plots of pooled contextualized embeddings of the TaxiNLI examples extracted from BERT and RoBERTA finetuned on MNLI with no retraining on the taxonomic labels. Color codes represent taxonomic categories (inset shows NLI categories: {\textbf{entailment}} (\mycbox{entailment}), \textbf{neutral} (\mycbox{neutral}), \textbf{contradiction} (\mycbox{contradiction})) and their combinations. Only combinations of up to two categories are included for brevity.
    % These layer-wise plots reveal the points along the neural processing stream where the clustering of various taxonomic categories starts to become identifiable. 
    % The smaller NLI label-overlay figures put the clustering of various taxonomic buckets into perspective by revealing the interaction between the two.
    % From L $\rightarrow$ R: 
    % (a,e) the {\tt \textcolor{yellow!50!red}{lexical}} bucket is revealed very early-on, even before any separation by NLI label; (b,f) the {\tt \textcolor{red!70!black}{syntactic}} and {\tt \textcolor{green!50!black}{logic}} buckets, as well as 
    % (c,g) the {\tt \textcolor{blue!80!black}{reasoning}} and {\tt \textcolor{blue!20!black}{knowledge}} buckets, are both observed about the same time as we see clustering by NLI labels;
    % (d,h) looking at all the categories together, we see a dominance of certain categories in the clusters by NLI label.
    }
    \label{fig:tsne}
\end{figure*}


  %The analysis in Sec~\ref{sec:eval} points out the differential performance of SOTA models in the various taxonomic categories. Re-affirming an increasing body of literature, it reminds us that despite rapid advancements in state-of-the-art techniques, the advancements are skewed, and happening faster along some dimensions
%(perhaps due to capitalizing on patterns or natural distributions of particular kinds of examples) 
%rather than all at once.

 %Instead of looking retroactively at how various models perform with respect to each taxonomic category, i
% Apart from post-facto category-wise error analysis, 
%% %% Where lies the difference?
%% %% do the systems acquire any information about what kind of reasoning is required, and is that represented in the <> space.
%% %% can it put them together?

\paragraph{Visual Analysis}
Section~\ref{sec:eval} paints a thorough picture by analysing the fine-grained capabilities of SOTA NLI systems at a \textit{behavioral}\footnote{
Similar to social sciences, as a black-box system} 
level. Whereas we can say the systems are lacking in certain aspects despite their high overall performance, it naturally also raises questions at the {\it understanding} level:
1) Is there any implicit knowledge acquired by the NLI-finetuned systems about the \textit{kinds} of reasoning required in the inference task? 2) If not, do the systems simply lack the understanding of what kind of reasoning is required per example, or despite understanding that, are unable to do the reasoning?
3) Can we make an argument for future work and model architecture that can more consciously use this information?

% It is also interesting to investigate whether the NLI models have implicit {\it a priori} of certain taxonomic categories, perhaps being utilized in the NLI task.
%Another growing body of literature tells us that Transformers learn different linguistic phenomena at different layers.
%There have been various probes, for instance, trying to understand where in the Transformers' processing stream syntactic knowledge is realized in the contextualized representations, with \citet{tenney2019bert,jawahar-etal-2019-bert} finding early evidence of syntactic knowledge, whereas \citet{liu2019linguistic} finding more delayed effects of syntax.
%% %% whether the knowledge is lacking? or whether it is implicitly present, but
% In light of the probing task literature \citet{tenney2019bert,jawahar-etal-2019-bert,liu2019linguistic} and the results from the Sec.~\ref{sec:eval},  we now ask the following: I) are there particular Transformer layers that are learning to tease out certain taxonomic categories, %which can give us insights into the differential performance of SOTA models across taxonomic categories, and, continuing the discussion started in Sec \ref{sec:confound}, 
% II) do certain taxonomic categories prevail for certain NLI labels, and what does that mean for the kind of progress happening in the task? %(for instance, how much can be gained by capitalizing on patterns or natural distributions of particular kinds of examples)?

In light of recent probing task literature \citep{tenney2019bert,jawahar-etal-2019-bert,liu2019linguistic}, we specifically investigate whether representations of examples cluster meaningfully into taxonomic categories relevant to the reasoning required for NLI.
We use the t-SNE \cite{maaten2008visualizing} algorithm to visualize pooled contextualized representations of NLI examples, under the lens of our taxonomy. For an NLI example, we construct the embeddings at a Transformer layer by
max-pooling hidden states over all input token positions concatenated with the {\tt [CLS]} token (typically used for classification tasks) representation.
% which is typically used for classification tasks. %, including NLI, in SOTA architectures (BERT-base, RoBERTa-large).
The resulting visualizations (Fig.~\ref{fig:tsne}) reveal definitive patterns of clustering by taxonomic categories. The earliest separation is observed for the {\tt lexical} category, at layer 3 in BERT (and layer 1 in RoBERTa), much before any other categories are realized.
% , or separation into NLI label clusters is observed. 
At layers 6 in BERT, and 19 in RoBERTa, about the same time as clustering by NLI label is seen, the \textit{connectives} cluster is revealed. The \textit{deductions} (see Sec.~\ref{sec:taxonomy}), and {\tt syntactic} categories are revealed in later layers (layer 11 and 12 in BERT and layer 21 in RoBERTa). The {\it knowledge} category is revealed more prominently in RoBERTa at layer 21, while BERT does not seem to show such a cluster.
By the last few layers, separation into most categories becomes apparent. This means, along various layers of a NLI finetuned language model, taxonomic information is implicitly captured. Despite this, as discussed in the previous sections, SOTA models seem to be deficient in some of the categories---certain categories remain harder to perform inference on.
% rhe discri ability is there, but for some of them 
In the latter layers, the separation along taxonomic categories also corresponds strongly with separation along NLI labels. For instance, in Fig.~\ref{fig:tsne} (c), the examples categorized as {\tt syntactic} almost entirely lie in the {\tt entailment} cloud, which matches our intuition based on the statstics in Fig.~\ref{fig:categories_freq}.

The layer-wise separation of examples by taxonomy raises an interesting possibility to motivate model architectures that may attempt to use its discriminative power to identify such taxonomic categories, for specialized treatment to examples requiring certain reasoning capabilities.
% For instance, it could apply a more robust logical process for examples requiring logic, or utilizing a knowledge base for examples that need to be grounded in the real world.

% reasoning --> deductions
% logic --> connective

%\paragraph{CheckList} Recently, \cite{ribeiro-etal-2020-beyond} listed a set of universal phenomena and suggested to adopt behavioral testing of NLP models. They noted a set of necessary capabilities for NLU systems: Vocabulary+POS, Taxonomy, NER, Temporal , Negation, Coreference, Semantic Role Labeling, and Logic (handling symmetry, consistency, and conjunctions).  Our categorization in-fact subsumes the inferencing categories, and our examples per categories \textsc{CheckList} can be thought of as templates for testing minimal functionality testing (MFT) conditions for the NLI task. 

% \begin{comment}

\textbf{Recasting: }
The under-representation of certain categories in the MNLI dataset raises a need for more balanced data collection. 
%As the distribution of categories are quite skewed across the datasets, there arises a need for balancing of categorical representation in training data. 
A possible alternative is to build recast diagnostic datasets for each category, and create probing tasks. Some datasets \cite{zhang-etal-2019-paws,probinglogical} can be recast to the \texttt{syntactic} and \textbf{\texttt{Logical}} categories respectively, as their data creation aligns with our category definitions. However, most categories lack such aligned synthetic data, and crowdsourced data would require manual annotation as above. %A solution is the careful selection and recasting of different NLU datasets.
%For example, certain datasets such as PAWS \cite{zhang-etal-2019-paws} and Logical Fragments \cite{probinglogical} can be recast to the \texttt{syntactic} and \textbf{\texttt{Logical}} categories respectively, provided that the data creation process aligns with our category definitions. %However, the challenges with this lie in how this can be done automatically or semi-automatically. 
%For other categories, such synthetically generated datasets are absent. Automatically recasting manually annotated datasets is challenging, since the linguistic variety may call for multiple labels for each example; warranting manual inspection. 
This poses an avenue for future work. %Coincidentally, our examples per category can be used as templates to generate synthetic minimal functionality tests (MFT) for NLI using the recently proposed \textsc{CheckList} system \cite{ribeiro-etal-2020-beyond}.

% \end{comment}

==> TaxiNLI 2020 10K/sections/7_conclusion.tex <==
\section{Conclusion}

%Observing the disparity between accuracy-led performance and linguistic analysis of the state-of-the-art, \citet{linzen-2020-accelerate} and \citet{bender-koller-2020-climbing} criticized the accuracy-led performance evaluation as an insufficient indicative task for tracking \textit{understanding}. Essentially, 
To bridge the gap between accuracy-led performance measurement and linguistic analysis of state-of-the-art NLI systems, we propose a taxonomic categorization of necessary inferencing capabilities for the NLI task, and a re-evaluation framework of systems on a re-annotated NLI dataset using this categorization; which underscores the reasoning categories that current systems struggle with.

We would like to emphasize that unlike the case with challenge and adversarial datasets, \textsc{TaxiNLI} re-annotates samples from existing NLI datasets which the SOTA models have been exposed to. Therefore, a lower accuracy in certain taxonomic categories in this case cannot be simply explained away by the ``lack of data" and ``unnatural distribution" arguments.
%\newpage

==> extra.tex <==
 \begin{table*}[!htpb]
  \resizebox{\textwidth}{!}{  
\begin{tabular}{|l|l|l|}
\hline
   & Synthetic Examples and Labels (E/C/N)                   & MNLI Examples and Labels (E/C/N)                                                                                                               \\ \hline
Lexical           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Anakin was compassionate. \\ H: Anakin was empathetic.\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: so it's stayed cold for the \underline{entire} week \\ H: It has been cold for the \underline{whole} week.\end{tabular} \\ \hline

Syntactic         & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Anakin was an excellent pilot. H: The \\ piloting skills of Anakin was as good as his \\singing.\end{tabular}                                           &   \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Those in Egypt, Libya, Iraq, and Yemen were \\eventually overthrown by secular nationalist revolutionaries.\\ H: Secular nationalist revolutionaries eventually \\overthrew them in Egypt and Libya.\end{tabular}                                                                                                                            \\ \hline
Factivity         &                                                                                                                                                                                         &                                                                                                                               \\ \hline
\multicolumn{3}{|c|}{\textbf{Logic}}                                                                                                                                                                                                                                                                                                                 \\ \hline\hline
Negation          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: Laurie has only visited Nephi, Marion has \\ only visited Calistoga. H:  Laurie didn’t visit \\ Calistoga.\end{tabular}                           &            \begin{tabular}[c]{@{}l@{}}{[}C{]} P: They \underline{post} loads of newspaper articles--Yahoo!\\ H:  Yahoo does \underline{not post} any articles from newspapers.\end{tabular}                                                                                                                   \\ \hline
Boolean           & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Travis, Arthur, Henry and Dan have only \\ visited Georgia. H:  Dan didn’t visit Rwanda.\end{tabular}                                             &     \begin{tabular}[c]{@{}l@{}}{[}E{]} P:According to contemporaneous notes, \\at 9:55 the Vice President was still on the phone with the\\ President advising that three planes were missing \underline{and} one had hit\\ the Pentagon.\\ H:  The President called the Vice President to \\tell him the plane hit the Pentagon.\end{tabular}                                                                                                                          \\ \hline
Quantifier        & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Everyone has visited every place. H:  Virgil \\ didn’t visit Barry.\end{tabular}                                                                  &   \begin{tabular}[c]{@{}l@{}}{[}C{]} P: \underline{Some} travelers add Molokai and Lanai to their itineraries.\\ H:  \underline{No one} decides to go toMolokai and Lanai.\end{tabular}                                                                                                                             \\ \hline
Conditionals      & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Francisco has  visited Potsdam and if \\Francisco  has visited Potsdam then Tyrone has \\ visited Pampa. H:  Tyrone has visited Pampa\end{tabular} & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Francisco has  visited Potsdam and if \\Francisco  has visited Potsdam then Tyrone has \\ visited Pampa. H:  Tyrone has visited Pampa\end{tabular}                                                                                                                              \\ \hline
Comparatives      & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: John \underline{is taller than} Gordon and Erik..., and \\ Mitchell is \underline{as tall as} John. H: Erik \underline{is taller than} \\ Gordon.\end{tabular}                        &      \begin{tabular}[c]{@{}l@{}}{[}N{]} P: Load time is divided into elemental and coverage related load time.\\ H: The coverage related load time \underline{is longer than} elemental.\end{tabular}                                                                                                                         \\ \hline
%Monotonicity      & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: All black mammals saw exactly 5 \\ stallions who  danced. H: A brown \\ poodle saw exactly 5 stallions who danced.\end{tabular}           &                                                                                                                               \\ \hline
\end{tabular}
}
\caption{We provide a synthetic example and an an example from MultiNLI dataset that fall in each categories. For a full set of examples and definitions, please look at appendix.}
\label{tabexamples}
\end{table*}

\begin{table*}[!htpb]
  \resizebox{\textwidth}{!}{  
\begin{tabular}{|l|l|l|}
\hline
                  & Synthetic Examples and Labels (E/C/N)                                                                                                                                                   & MNLI Examples and Labels (E/C/N)                                                                                                               \\ \hline
    \multicolumn{3}{|c|}{\textbf{Reasoning}}                                                                       \\ \hline\hline
Relational        & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: \underline{Jack} and his \underline{brother} played cards. \\ H: The \underline{two siblings} played cards..\end{tabular}                                                             &   \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Actually, \underline{my sister} wrote a story on it. \\ H: \underline{My sibling} created a story about it. \end{tabular}                                                                                                                                                                  \\ \hline
Spatial  & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: The restaurant is just left of the shop,\\ opposite  the apartments. H: The restaurant is \\next to the shop.\end{tabular}                          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: At the eastern end of Back Lane and turning right,\\ Nicholas Street becomes Patrick Street, and in St. Patrick's\\ Close is St. Patrick's Cathedral .\\ H: Nicholas Street becomes Patrick Street after\\ turning left at the eastern end of Back Lane.\end{tabular}                                                                                                                              \\ \hline
Temporal          & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: They worked in the fields only between\\ 3:30pm  and 4:40pm. H: They were hard at work \\ in the fields at 7:00pm.\end{tabular}                   &  \begin{tabular}[c]{@{}l@{}}{[}C{]} P: See you \underline{Aug. 12, or soon thereafter}, we hope.\\ H: The person told not to come \underline{until December}.\end{tabular}                                                                                                                             \\ \hline
Coreference       & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Jack found James annoying because of \\\underline{his}  constant meddling. H: \underline{Jack} was constantly \\ meddling with James\end{tabular}                         &    \begin{tabular}[c]{@{}l@{}}{[}E{]} P: Acroseon the mountainside is another terrace on which \\imperial courtiers and dignitaries would sit while \\enjoying dance performances and music recitals on the \underline{hondo's broad terrace}.\\ H: There is a \underline{terrace} where musicians play.\end{tabular}                                                                                                                           \\ \hline
Causality       &\begin{tabular}[c]{@{}l@{}}{[}E{]} P:  John shot Mia in the leg. \\ H:Mia is hurt.\end{tabular}                                                                                                                              & \begin{tabular}[c]{@{}l@{}}{[}N{]} P: A dozen minor wounds crossed his forearms and body. \\ H: The grenade explosion left him with a lot of wounds.\end{tabular}                                                                                                                               \\ \hline
\multicolumn{3}{|c|}{\textbf{Knowledge}}                                                                      \\ \hline\hline
World             & \begin{tabular}[c]{@{}l@{}}{[}C{]} P: The church gathered in prayer. H: They \\ prayed to Allah.\end{tabular}                                                                           &                                                                                           
 \\ \hline
Taxonomic         & \begin{tabular}[c]{@{}l@{}}{[}E{]} P: The ladybug ate part of the rose. \\ H: The insect ate part of the flower.\end{tabular}                                                           &                                                                                  \\ \hline   
\end{tabular}
}
\caption{In this table, we provide examples for the Reaosning and Knowledge categories. For a full set of examples and definitions, please look at appendix.}
\label{tabexamples2}
\end{table*}
